I/O in Machine Learning Applications on HPC Systems: A 360-degree Survey

Growing interest in Artificial Intelligence (AI) has resulted in a surge in demand for faster methods of Machine Learning (ML) model training and inference. This demand for speed has prompted the use of high performance computing (HPC) systems that excel in managing distributed workloads. Because data is the main fuel for AI applications, the performance of the storage and I/O subsystem of HPC systems is critical. In the past, HPC applications accessed large portions of data written by simulations or experiments or ingested data for visualizations or analysis tasks. ML workloads perform small reads spread across a large number of random files. This shift of I/O access patterns poses several challenges to modern parallel storage systems. In this paper, we survey I/O in ML applications on HPC systems, and target literature within a 6-year time window from 2019 to 2024. We define the scope of the survey, provide an overview of the common phases of ML, review available profilers and benchmarks, examine the I/O patterns encountered during offline data preparation, training, and inference, and explore I/O optimizations utilized in modern ML frameworks and proposed in recent literature. Lastly, we seek to expose research gaps that could spawn further R&D

==> tables/comparison.tex <==
\begin{table}[]
\centering
\small
%\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccccc}
\multicolumn{2}{l}{\textbf{Features}}          & \textbf{PDC} & \textbf{\begin{tabular}[c]{@{}c@{}}AWS\\ S3\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}OpenStack\\ (swift)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Google Cloud\\ Storage\end{tabular}} & \textbf{CEPH} & \textbf{DAOS} & \textbf{ADIOS} & \textbf{HDF5} \\
\toprule
%\multicolumn{2}{l}{\textbf{Interfaces}}        & C API        & SDK, REST API, CLI & REST API, CLI              & SDK, REST API, CLI            & SDK, REST API & SDK           & SDK            & SDK, REST API \\
%\midrule
\multicolumn{2}{l}{\textbf{HPC oriented}}      & \YES         & \NO              & \NO                      & \NO                         & \NO         & \YES          & \YES           & \YES          \\
\midrule
\multicolumn{2}{l}{\textbf{Group abstraction}} & Containers   & Buckets            & Containers                 & Buckets                       & Buckets       & Containers    & -              & Groups        \\
                & Management                   & \YES         & \YES               & \YES                       & \YES                          & \YES          & \YES          & \NO          & \YES          \\
                & Lifecycle                    & \YES         & \YES               & \NO                      & \YES                          & \YES          & \NO         & \NO          & \NO         \\
                & Tagging                      & \YES         & \YES               & \YES                       & \YES                          & \MAYBE          & \YES          & \NO          & \YES          \\
                & Encryption                   & \NO        & \YES               & \YES                       & \NO                         & \NO         & \NO         & \NO          & \NO         \\
                & Versioning                   & \NO        & \YES               & \YES                       & \YES                          & \YES          & \NO         & \NO          & \NO         \\
\midrule
\multicolumn{2}{l}{\textbf{Data abstraction}}  & Objects      & Objects            & Objects                    & Objects                       & Objects       & Objects       & Objects        & Datasets      \\
                & Management                   & \YES         & \YES               & \YES                       & \YES                          & \YES          & \YES          & \YES           & \YES          \\
                & Collectiveness               & \YES         & \NO              & \NO                      & \NO                         & \NO         & \YES          & \YES           & \YES          \\
                & Multipart                    & \NO        & \YES               & \YES                       & \YES                          & \YES          & \NO         & \NO          & \NO         \\
                & Tagging                      & \YES         & \YES               & \YES                       & \NO                         & \YES          & \NO         & \NO          & \YES          \\
\midrule
\multicolumn{2}{l}{\textbf{Querying}}          & \YES         & \YES               & \MAYBE                       & \MAYBE                          & \YES          & \NO         & \NO          & \NO         \\
\midrule
\multicolumn{2}{l}{\textbf{Transformations}}   & \YES         & \YES               & \MAYBE                       & \YES                          & \MAYBE          & \NO         & \NO          & \NO \\
\midrule
\multicolumn{2}{l}{\textbf{REST API}}          & \NO        & \YES               & \YES                       & \YES                          & \YES          & \NO         & \NO          & \YES          \\
\bottomrule
\end{tabular}
%}
\caption{Summary of features exposed by interfaces and APIs of different object storage solutions.}
\label{table:summary-features-solutions}
\end{table}

==> tables/datasets.tex <==
\begin{table}[htbp]
    \centering
    \begin{tabular}{lccc}
        \toprule
        Dataset Modality & Total Files & Total Dataset Size & File Formats Used \\
        \midrule
        Image Datasets & & & \\
        \midrule
        MNIST \cite{mnist-dataset} & $4$ & $101.16$ MiB & Custom \\
        CIFAR-100 \cite{cifar-dataset} & $60000$ & $184$ MiB & Custom \\
        ImageNet \cite{imagenet-a-large-scale-heirarchical-image-database} & $1,431,167$ & $150$ GiB & JPEG, TXT \\
        \midrule
        Audio Datasets & & & \\
        \midrule
        UrbanSound8K \cite{urbansound-dataset} & $18733$ & $6.60$ GiB & WAV, CSV \\
        LibriSpeech \cite{librispeech} & $10,000$ & $60$ GiB & FLAC, TXT \\
        AudioSet \cite{audioset-dataset} & $2,084,320$ & $2.4$ GiB & TFRecord, CSV \\
        \midrule
        Video Datasets & & & \\
        \midrule
        Charades \cite{charades-dataset} & $9,900$ & $55$ GiB & CSV, TXT, MATLAB, JPEG Frames \\
        UCF101 \cite{ufc101} & $13,320$ & $6.69$ GiB & AVI \\
        HMDB \cite{hmdb-dataset} & $7,000$ & $2$ GiB & TXT, AVI  \\
        \midrule
        Time Series Datasets & & & \\
        \midrule
        NAB \cite{nab-dataset} & $58$ & $9$ MiB & CSV \\
        M4 \cite{m4-dataset} & $13$ & $310$ MiB & CSV \\
        UCR Time Series Archive \cite{ucr-dataset} & $416$ & $853$ MiB & TSV \\
        \midrule
        Graph Datasets & & & \\
        \midrule
        Cora \cite{cora-dataset} & $1$ & $270$ KiB & CSV \\
        Protein-Protein Int. \cite{protein-dataset} & $1$ & $3,661$ KiB & CSV \\
        Amazon Co-purchasing \cite{amazon-dataset} & $1$ & $954,597$ KiB & TXT \\
        \bottomrule
    \end{tabular}
    \vspace{5pt}
    \caption{Comparison of different ML dataset modalities}
    \label{tab:ml_dataset_comparison}
\end{table}

==> tables/traditional-hpc-interfaces.tex <==
\begin{table}[]

\centering
\small
\begin{tabular}{cm{6cm}m{6cm}}
    \textbf{Interface} 
            & \textbf{Opportunities}
                & \textbf{Challenges}   \\
    \toprule
    \textbf{POSIX}
            & 
            \begin{minipage}[t]{\linewidth}
                \begin{itemize}[nosep, wide=0pt]
                    \item Portability
                    \item Strong consistency guarantees
                    \item Shallow learning curve (wide adoption)
                \end{itemize}
            \end{minipage}
            &
            \begin{minipage}[t]{\linewidth}
                \begin{itemize}[nosep, wide=0pt]
                    \item Not designed for HPC
                    \item Strong consistency vs. scalability
                    \item Collective access (locking)
                    \item Optimizations (lack of whole application view)
                \end{itemize}
            \end{minipage} \\
    \midrule
    \textbf{MPI-IO}
            &
            \begin{minipage}[t]{\linewidth}
                \begin{itemize}[nosep, wide=0pt, after=\strut]
                    \item Designed for HPC
                    \item Relaxed consistency
                    \item Flexibility (express patterns natural to applications)
                    \item High-level I/O optimizations
                \end{itemize} 
            \end{minipage}
            & 
            \begin{minipage}[t]{\linewidth}
                \begin{itemize}[nosep, wide=0pt, after=\strut]
                    \item Hard adoption (source-code changes)
                    \item Complex tunning
                \end{itemize}
            \end{minipage} \\
    \midrule
    \textbf{STDIO}
            &
            \begin{minipage}[t]{\linewidth}
                \begin{itemize}[nosep, wide=0pt]
                    \item Simple and buffered stream interface
                \end{itemize}
            \end{minipage}
            & 
            \begin{minipage}[t]{\linewidth}
                \begin{itemize}[nosep, wide=0pt]
                    \item Not designed for HPC
                    \item Scalability
                    \item Optimizations (lack of whole application view)
                \end{itemize}
            \end{minipage} \\
    \bottomrule
\end{tabular}
\caption{Opportunities and challenges presented by traditional I/O interfaces when used in HPC.}
\label{tab:interfaces-pros-cons}
\end{table}
